Constraint-based Diversification of JOP Gadgets

Modern software deployment process produces software that is uniform and hence vulnerable to large-scale code-reuse attacks, such as Jump-Oriented Programming (JOP) attacks. Compiler-based diversification improves the resilience of software systems by automatically generating different assembly code versions of a given program. Existing techniques are efficient but do not have a precise control over the quality of the generated variants. This paper introduces Diversity by Construction (DivCon), a constraint-based approach to software diversification. Unlike previous approaches, DivCon allows users to control and adjust the conflicting goals of diversity and code quality. A key enabler is the use of Large Neighborhood Search (LNS) to generate highly diverse code efficiently. For larger problems, we propose a combination of LNS with a structural decomposition of the problem. To further improve the diversification efficiency of DivCon against JOP attacks, we propose an application-specific distance measure tailored to the characteristics of JOP attacks. We evaluate DivCon with 20 functions from a popular benchmark suite for embedded systems. These experiments show that the combination of LNS and our application-specific distance measure generates binary programs that are highly resilient against JOP attacks. Our results confirm that there is a trade-off between the quality of each assembly code version and the diversity of the entire pool of versions. In particular, the experiments show that DivCon generates near-optimal binary programs that share a small number of gadgets. For constraint programming researchers and practitioners, this paper demonstrates that LNS is a valuable technique for finding diverse solutions. For security researchers and software engineers, DivCon extends the scope of compiler-based diversification to performance-critical and resource-constrained applications.

==> tables/benchmarks.tex <==
\begin{longtable}{|l|l|l|l|l|}
\caption{\label{tab:benchmarks}{Benchmark functions}}\\
\hline
{ID}&{app}&{function name}&{b}&{i}\\
\hline
b1&sphinx3&ptmr\_init&1&10
\\
b2&gcc&ceil\_log2&1&14
\\
b3&mesa&glIndexd&1&14
\\
b4&h264ref&symbol2uvlc&1&15
\\
b5&gobmk&autohelperowl\_defen..&1&23
\\
b6&mesa&glVertex2i&1&23
\\
b7&hmmer&AllocFancyAli&1&25
\\
b8&gobmk&autohelperowl\_vital..&1&27
\\
b9&gobmk&autohelperpat1088&1&29
\\
b10&gobmk&autohelperowl\_attac..&1&30
\\
b11&gobmk&get\_last\_player&3&13
\\
b12&h264ref&UpdateRandomAccess&3&16
\\
b13&gcc&xexit&3&17
\\
b14&gcc&unsigned\_condition&3&24
\\
b15&sphinx3&glist\_tail&4&10
\\
b16&gcc&get\_frame\_alias\_set&5&20
\\
b17&gcc&parms\_set&5&25
\\
\hline
\end{longtable}


==> tables/decomp_gaps.tex <==
\begin{longtable}{|l|c|c|c|c|c|c|c|c|}
\caption{\label{tab:agaps} Trade-off between Diversity and Optimality}\\
\hline
\multirow{2}{*}{ID}&\multicolumn{2}{c|}{0\%}&\multicolumn{2}{c|}{5\%}&\multicolumn{2}{c|}{10\%}&\multicolumn{2}{c|}{20\%}\\
\cline{2-9}
&$d$&num&$d$&num&$d$&num&$d$&num\\
\hline
b1&7.5$\pm$0.3 & 200&\textbf{9.0$\pm$1.1} & 200&\textbf{9.7$\pm$1.3} & 200&\textbf{9.4$\pm$1.6} & 200
\\
b2&\textbf{9.1$\pm$1.2} & 200&\textbf{9.6$\pm$1.4} & 200&\textbf{9.8$\pm$1.9} & 200&\textbf{9.7$\pm$1.9} & 200
\\
b3&15.3$\pm$0.2 & 200&19.9$\pm$0.4 & 200&22.0$\pm$1.0 & 200&\textbf{23.5$\pm$2.2} & 200
\\
b4&\textit{4.9$\pm$1.2} & 11&\textbf{11.8$\pm$1.8} & 200&\textbf{12.2$\pm$1.4} & 200&\textbf{12.2$\pm$1.8} & 200
\\
b5&\textit{2.0$\pm$0.0} & 28&8.8$\pm$1.0 & 200&\textbf{11.8$\pm$1.9} & 200&10.7$\pm$2.4 & 200
\\
b6&4.3$\pm$0.0 & 200&\textbf{12.9$\pm$0.9} & 200&\textbf{13.1$\pm$1.6} & 200&\textbf{13.1$\pm$1.8} & 200
\\
b7&10.1$\pm$0.9 & 200&21.0$\pm$4.8 & 200&19.8$\pm$4.9 & 200&\textbf{22.9$\pm$6.0} & 200
\\
b8&10.7$\pm$1.2 & 200&24.7$\pm$5.5 & 200&25.6$\pm$5.6 & 200&\textbf{30.1$\pm$6.9} & 200
\\
b9&16.5$\pm$3.2 & 200&\textbf{34.0$\pm$14.8} & 200&30.6$\pm$14.4 & 200&\textbf{33.4$\pm$12.5} & 200
\\
b10&10.4$\pm$1.2 & 200&\textbf{30.5$\pm$8.0} & 200&28.1$\pm$6.8 & 200&\textbf{30.9$\pm$5.8} & 200
\\
b11&13.9$\pm$2.5 & 200&31.2$\pm$15.8 & 200&32.1$\pm$15.0 & 200&\textbf{43.6$\pm$16.8} & 200
\\
b12&17.9$\pm$3.9 & 200&34.7$\pm$20.1 & 200&36.6$\pm$20.5 & 200&\textbf{38.2$\pm$20.5} & 200
\\
b13&17.0$\pm$3.5 & 200&35.6$\pm$8.5 & 200&49.3$\pm$13.6 & 200&\textbf{51.3$\pm$14.2} & 200
\\
b14&11.4$\pm$1.0 & 200&44.1$\pm$7.4 & 200&47.6$\pm$11.0 & 200&\textbf{61.1$\pm$12.3} & 200
\\
\hline
\end{longtable}


==> tables/lns_gaps_only_d.tex <==
\begin{longtable}{|l|c|c|c|c|c|c|c|c|}
\caption{\label{tab:agaps} Trade-off between Diversity and Optimality}\\
\hline
\multirow{2}{*}{ID}&\multicolumn{2}{c|}{0\%}&\multicolumn{2}{c|}{5\%}&\multicolumn{2}{c|}{10\%}&\multicolumn{2}{c|}{20\%}\\
\cline{2-9}
&$d$&num&$d$&num&$d$&num&$d$&num\\
\hline
b1&7.7$\pm$0.1 & 200&11.1$\pm$0.9 & 200&13.2$\pm$0.6 & 200&\textbf{17.5$\pm$1.3} & 200
\\
b2&10.6$\pm$0.1 & 200&13.8$\pm$1.5 & 200&14.8$\pm$1.1 & 200&\textbf{19.0$\pm$1.1} & 200
\\
b3&15.7$\pm$0.0 & 200&19.6$\pm$0.8 & 200&23.5$\pm$0.8 & 200&\textbf{28.8$\pm$1.1} & 200
\\
b4&7.2$\pm$0.3 & 200&22.0$\pm$8.7 & 200&26.6$\pm$6.6 & 200&\textbf{32.9$\pm$2.1} & 200
\\
b5&\textit{2.7$\pm$0.0} & 4&9.7$\pm$1.2 & 200&15.4$\pm$1.4 & 200&\textbf{19.6$\pm$2.2} & 200
\\
b6&\textit{4.4$\pm$0.0} & 32&16.5$\pm$3.9 & 200&22.8$\pm$2.3 & 200&\textbf{32.8$\pm$2.3} & 200
\\
b7&14.6$\pm$0.3 & 200&39.2$\pm$3.2 & 200&45.2$\pm$2.4 & 200&\textbf{50.7$\pm$3.5} & 200
\\
b8&19.1$\pm$0.5 & 200&50.0$\pm$3.3 & 200&57.4$\pm$3.0 & 200&\textbf{66.1$\pm$2.4} & 200
\\
b9&41.6$\pm$0.9 & 200&150.4$\pm$17.0 & 200&160.9$\pm$16.0 & 200&\textbf{178.2$\pm$11.9} & 200
\\
b10&13.8$\pm$0.2 & 200&57.9$\pm$5.1 & 200&64.0$\pm$7.2 & 200&\textbf{76.0$\pm$2.2} & 200
\\
b11&52.9$\pm$0.7 & 200&115.6$\pm$3.0 & 200&127.4$\pm$3.7 & 200&\textbf{142.8$\pm$2.7} & 200
\\
b12&\textit{81.9$\pm$26.1} & 163&\textit{127.1$\pm$3.1} & 142&\textit{136.1$\pm$2.6} & 154&\textit{159.2$\pm$3.9} & 184
\\
b13&83.1$\pm$24.9 & 200&137.8$\pm$3.0 & 200&155.9$\pm$4.4 & 200&\textbf{180.2$\pm$11.4} & 200
\\
b14&25.6$\pm$0.5 & 200&84.4$\pm$5.9 & 200&103.7$\pm$5.4 & 200&\textbf{133.5$\pm$4.8} & 200
\\
\hline
\end{longtable}


==> tables/merge_different_res.tex <==
\begin{longtable}{|l|c|c|c|c|c|c|}
\caption{\label{tab:decomp}{Comparison between RS and DMLNS}}\\
\hline
\multirow{2}{*}{ID}&\multicolumn{2}{c|}{DFS}&\multicolumn{2}{c|}{LNS}&\multicolumn{2}{c|}{DMLNS}\\
\cline{2-7}
&$t(s)$&num&$t(s)$&num&$t(s)$&num\\
\hline
b1&0.2$\pm$0.0 & 5.7$\pm$0.1 (200)&2.4$\pm$0.7 & 14.0$\pm$0.4 (200)&11.8$\pm$3.3 & 10.5$\pm$1.4 (200)
\\                                                                 
b2&0.2$\pm$0.0 & 5.2$\pm$0.1 (200)&2.2$\pm$1.0 & 16.1$\pm$0.7 (200)&6.2$\pm$1.3 & 9.8$\pm$1.9 (200)
\\                                                                 
b3&0.4$\pm$0.0 & 4.5$\pm$0.0 (200)&92.9$\pm$18.5 & 24.7$\pm$0.5 (200)&101.9$\pm$27.7 & 23.1$\pm$0.9 (200)
\\                                                                 
b4&0.1$\pm$0.0 & 4.0$\pm$0.3 (200)&9.2$\pm$6.0 & 30.1$\pm$1.7 (200)&8.9$\pm$5.1 & 12.1$\pm$1.9 (200)
\\                                                                 
b5&0.2$\pm$0.0 & 5.3$\pm$0.0 (200)&1.2$\pm$0.0 & 16.7$\pm$1.3 (200)&10.0$\pm$6.0 & 11.6$\pm$1.8 (200)
\\                                                                 
b6&0.2$\pm$0.0 & 5.3$\pm$0.1 (200)&10.6$\pm$2.0 & 26.9$\pm$1.6 (200)&5.7$\pm$1.3 & 12.7$\pm$1.7 (200)
\\                                                                
b7&0.4$\pm$0.0 & 4.9$\pm$0.1 (200)&33.1$\pm$13.5 & 47.3$\pm$2.5 (200)&4.2$\pm$0.9 & 20.1$\pm$5.3 (200)
\\                                                                 
b8&0.5$\pm$0.0 & 4.2$\pm$0.2 (200)&42.9$\pm$7.9 & 60.8$\pm$2.6 (200&4.4$\pm$0.6 & 24.6$\pm$6.3 (200)
\\
b9&- & -&- & -&8.0$\pm$1.0 & 39.9$\pm$9.6 (200)
\\
b10&0.7$\pm$0.0 & 3.0$\pm$0.0 (200)&121.3$\pm$21.6 & 74.3$\pm$2.1 (200)&6.2$\pm$2.1 & 27.2$\pm$7.0 (200)
\\                                 
b11&4.7$\pm$0.9 & 1.7$\pm$0.0 (200)&- & -&6.5$\pm$0.4 & 40.2$\pm$14.1 (200)
\\                                 
b12&6.1$\pm$0.0 & 1.2$\pm$0.0 (200)&- & -&7.7$\pm$0.6 & 45.2$\pm$16.5 (200)
\\                                 
b13&8.0$\pm$0.4 & 1.9$\pm$0.0 (200)&\textit{436.8$\pm$108.6} & \textit{144.5$\pm$10.6 (200)}&8.3$\pm$1.5 & 46.1$\pm$14.0 (200)
\\                                                                                          
b14&3.1$\pm$0.1 & 1.9$\pm$0.0 (200)&\textit{455.9$\pm$100.9} & \textit{97.7$\pm$12.2 (200)}&8.3$\pm$0.5 & 50.1$\pm$6.4 (200)
\\
\hline
\end{longtable}

